Characterizing Financial Market Coverage using Artificial Intelligence

This paper scrutinizes a database of over 4900 YouTube videos to characterize financial market coverage. Financial market coverage generates a large number of videos. Therefore, watching these videos to derive actionable insights could be challenging and complex. In this paper, we leverage Whisper, a speech-to-text model from OpenAI, to generate a text corpus of market coverage videos from Bloomberg and Yahoo Finance. We employ natural language processing to extract insights regarding language use from the market coverage. Moreover, we examine the prominent presence of trending topics and their evolution over time, and the impacts that some individuals and organizations have on the financial market. Our characterization highlights the dynamics of the financial market coverage and provides valuable insights reflecting broad discussions regarding recent financial events and the world economy.

==> moule.tex <==
Yahoo Finance stock coverage

Yahoo Finance-like medias' stock coverage

%- Tasks: identify these aforementioned actors and copy manually the links of coverage in a text file with their dates.

- Contribution: using whisper to extract datasets and make them open 

- One of first works to compare the narratives between reliable medias and individuals. -- The advantage: zero bot with the dataset.


Most studies XXX financial news, social media news (using verified and regular accounts), conduct market coverage...; some data from social media are price oriented, but XXX media coverage are factual oriented and decrypt market news and events to help people understand XXX

The advantages for analyzing : viewpoints from renowned experts and real-time coverage where they can get contradicted... zero bots, reliable content generated by experts... The release of the OpenAI Whisper model comes to facilitate the XXX

\textbf{tedious to analyze}

{\bf Market coverage generate large volumes of video data. Listening to tons of market coverage videos to derive actionable insights can be challenging and complex.}\\\


{\bf The purpose of this work is to xxx}


\noindent
\textbf{Background and Related Works:} XXX XXX XXX XXX XXX \\\\\

\noindent
\textbf{Major Contributions:} XXX XXX XXX XXX XXX \\\


